Assessing Differentially Private Variational Autoencoders under Membership Inference

We present an approach to quantify and compare the privacy-accuracy trade-off for differentially private Variational Autoencoders. Our work complements previous work in two aspects. First, we evaluate the the strong reconstruction MI attack against Variational Autoencoders under differential privacy. Second, we address the data scientist's challenge of setting privacy parameter epsilon, which steers the differential privacy strength and thus also the privacy-accuracy trade-off. In our experimental study we consider image and time series data, and three local and central differential privacy mechanisms. We find that the privacy-accuracy trade-offs strongly depend on the dataset and model architecture. We do rarely observe favorable privacy-accuracy trade-off for Variational Autoencoders, and identify a case where LDP outperforms CDP.

==> defi.tex <==
%%custom packages
% Magic hack for subcaption and svg compatibility
% https://tex.stackexchange.com/questions/291929/svg-package-and-subcaption-incompability
\RequirePackage{scrlfile}
\PreventPackageFromLoading{subfig}

\usepackage[inline]{enumitem}
\usepackage{comment}
%\usepackage{cite}
\usepackage{todonotes}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol} 
%\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{hyperref}
%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm}
\usepackage{tikz}
\usepackage{pdfpages}
\usepackage{tabularx}
\usepackage{mathrsfs}
\usepackage{amsmath,amstext,amssymb}
%\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[thinc]{esdiff}
\usepackage{xspace}
\usepackage{adjustbox}

\usepackage{balance}
\usepackage{microtype}
\usepackage{cryptocode}
\usepackage{makecell}


\usetikzlibrary{shapes, fit}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}

\usepackage{url}
\usepackage{textcomp}
\usepackage{color}
\graphicspath{{figures/}}
%% Custom definitions
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\feps}{\ensuremath{\epsilon'}\xspace}
\newcommand{\dlt}{\ensuremath{\delta}\xspace}
\newcommand{\sgm}{\ensuremath{\sigma}\xspace}
\newcommand{\tht}{\ensuremath{\theta}\xspace}
\newcommand{\epsdlt}{\ensuremath{(\epsilon,\delta)}\xspace}
\newcommand{\money}[1]{\$#1}
\newcommand{\person}[1]{\textsc{#1}}
\newcommand{\cali}[1]{\ensuremath{\mathcal{#1}}} % for uppercase letters only
\newcommand{\var}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\varbf}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\subscr}[2]{\ensuremath{#1_{\var{#2}}}}
\newcommand{\supscr}[2]{\ensuremath{#1^{\var{#2}}}}
\newcommand{\subsup}[3]{\ensuremath{#1_{\var{#2}}^{\var{#3}}}}
\newcommand{\pprime}{\ensuremath{\prime}}
\newcommand{\filenamename}{\edef\foo{\currfilebase}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\Z}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\N}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}\xspace}

\newcommand{\Ami}{\mathcal{A}_{\var{MI}}}
\newcommand{\Astrong}{\mathcal{A}_{\var{DI}}}
\newcommand{\AstrongGau}{\mathcal{A}_{\var{DI, Gau}}}

\newcommand{\datapoint}{x}

\newcommand{\madi}{\mathrm{Adv}^{\mathrm{DI}}}
\newcommand{\madiGau}{\mathrm{Adv}^{\mathrm{DI, Gau}}}
\newcommand{\mami}{\mathrm{Adv}^{\mathrm{MI}}}

\newcommand{\edi}{\mathrm{Exp}^{\mathrm{DI}}}
\newcommand{\emi}{\mathrm{Exp}^{\mathrm{MI}}}

\newcommand{\ra}{\mathrm{\rho}_{\mathrm{\alpha}}}
\newcommand{\rb}{\mathrm{\rho}_{\mathrm{\beta}}}

\newcommand{\dpgrad}{\ensuremath{\tilde g}\xspace}
%clippedgrad
\newcommand{\clgrad}{\ensuremath{\hat{g}}\xspace}

\newcommand{\sens}{\ensuremath{\Delta f}\xspace}

\newcommand{\clip}{\ensuremath{\var{C}}\xspace}

% uncomment for IEEE / comment for ACM
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}

%\newtheoremstyle{defistyle}% name für den Stil
%
%  {}%      Space above
%
%  {}%      Space below
%
%  {\itshape}%      Body font
%
%  {}%      Indent amount (empty = no indent, \parindent = para indent)
%
%  {\bfseries\sffamily}% Thm head font
%
%  {\rm.}%        Punctuation after thm head
%
%  { }% Space after thm head: " " = normal interword space; \newline = linebreak
%
%  {} %{\textbf{\thmname{Definition}} (\thmnote{#3})}%         Thm head spec (can be left empty, meaning `normal')
%
%  % http://www.stat.umn.edu/~charlie/amslatex.html <http://www.stat.umn.edu/~charlie/amslatex.html> 
%
%\theoremstyle{defistyle}

% quotes

\newcommand{\bq}{``}

\newcommand{\red}[1]{\textcolor{black}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\revised}[1]{\textcolor{blue}{#1}}

\newcommand{\eq}{''}

\newcommand{\q}[1]{\bq{#1}\eq}

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\Rkk}{R_{k}}

\let\oldReturn\Return
\renewcommand{\Return}{\State\oldReturn}

\newif\iffullversion
\fullversionfalse

==> figures/CDP_phi.tex <==
\begin{figure}[ht]
	\centering
    \begin{tabular}{c}
		\begin{subfigure}{0.45\linewidth}
            \includegraphics[width=\linewidth]{fig/lfw20_CDP_phi_over_noise.pdf}\\ 
        	\subcaption{LFW20.}
        	\label{fig:discussion:cdp:phi:lfw}
        \end{subfigure}
        \hfill
    	\begin{subfigure}{0.45\linewidth}
            	\includegraphics[width=\linewidth]{fig/ms_CDP_phi_over_noise.pdf}\\
    	    \subcaption{MotionSense.}
    	    \label{fig:discussion:cdp:phi:ms}
    	\end{subfigure}
    	\\
	\footnotesize\sffamily\textbf{Source:} \textit{custom figures}
	\end{tabular}
	\caption{Development of $\varphi$ for different noise multiplier $z$ for the CDP experiment.}
	\label{fig:discussion:cdp:phi}
\end{figure}

==> figures/LDP_phi.tex <==
\begin{figure}[ht]
	\centering
    \begin{tabular}{c}
		\begin{subfigure}{0.45\linewidth}
            \includegraphics[width=\linewidth]{fig/lfw20_LDP_train_phi_over_noise.pdf}\\ 
        	\subcaption{LFW20 train.}
        	\label{fig:discussion:ldptrain:phi:lfw}
        \end{subfigure}
        \hfill
    	\begin{subfigure}{0.45\linewidth}
            	\includegraphics[width=\linewidth]{fig/ms_LDP_train_phi_over_noise.pdf}\\
    	    \subcaption{MotionSense train.}
    	    \label{fig:discussion:ldptrain:phi:ms}
    	\end{subfigure}
    	\\
		\begin{subfigure}{0.45\linewidth}
            \includegraphics[width=\linewidth]{fig/lfw20_LDP_full_phi_over_noise.pdf}\\ 
        	\subcaption{LFW20 full.}
        	\label{fig:discussion:ldpfull:phi:lfw}
        \end{subfigure}
        \hfill
    	\begin{subfigure}{0.45\linewidth}
            	\includegraphics[width=\linewidth]{fig/ms_LDP_full_phi_over_noise.pdf}\\
    	    \subcaption{MotionSense full.}
    	    \label{fig:discussion:ldpfull:phi:ms}
    	\end{subfigure}
    	\\
	\footnotesize\sffamily\textbf{Source:} \textit{custom figures}
	\end{tabular}
	\caption{Development of $\varphi$ for different privacy parameters $\eps_i$ for the LDP experiment.}
	\label{fig:discussion:ldp:phi}
\end{figure}

==> figures/VAELDP_phi.tex <==
\begin{figure}[ht]
	\centering
    \begin{tabular}{c}
		\begin{subfigure}{0.45\linewidth}
            \includegraphics[width=\linewidth]{fig/lfw20_VAE-LDP_train_phi_over_noise.pdf}\\ 
        	\subcaption{LFW20 train.}
        	\label{fig:discussion:vaeldptrain:phi:lfw}
        \end{subfigure}
        \hfill
    	\begin{subfigure}{0.45\linewidth}
            	\includegraphics[width=\linewidth]{fig/ms_VAE-LDP_train_phi_over_noise.pdf}\\
    	    \subcaption{MotionSense train.}
    	    \label{fig:discussion:vaeldptrain:phi:ms}
    	\end{subfigure}
    	\\
		\begin{subfigure}{0.45\linewidth}
            \includegraphics[width=\linewidth]{fig/lfw20_VAE-LDP_full_phi_over_noise.pdf}\\ 
        	\subcaption{LFW20 full.}
        	\label{fig:discussion:vaeldpfull:phi:lfw}
        \end{subfigure}
        \hfill
    	\begin{subfigure}{0.45\linewidth}
            	\includegraphics[width=\linewidth]{fig/ms_VAE-LDP_full_phi_over_noise.pdf}\\
    	    \subcaption{MotionSense full.}
    	    \label{fig:discussion:vaeldpfull:phi:ms}
    	\end{subfigure}
    	\\
	\footnotesize\sffamily\textbf{Source:} \textit{custom figures}
	\end{tabular}
	\caption{Development of $\varphi$ for different noise bounds $\sigma$ for the VAE-LDP experiment.}
	\label{fig:discussion:vaeldp:phi}
\end{figure}
